The Rate-Distortion-Perception Trade-off with Side Information

In image compression, with recent advances in generative modeling, the existence of a trade-off between the rate and the perceptual quality has been brought to light, where the perception is measured by the closeness of the output distribution to the source. This leads to the question: how does a perception constraint impact the trade-off between the rate and traditional distortion constraints, typically quantified by a single-letter distortion measure? We consider the compression of a memoryless source $X$ in the presence of memoryless side information $Z,$ studied by Wyner and Ziv, but elucidate the impact of a perfect realism constraint, which requires the output distribution to match the source distribution. We consider two cases: when $Z$ is available only at the decoder or at both the encoder and the decoder. The rate-distortion trade-off with perfect realism is characterized for sources on general alphabets when infinite common randomness is available between the encoder and the decoder. We show that, similarly to traditional source coding with side information, the two cases are equivalent when $X$ and $Z$ are jointly Gaussian under the squared error distortion measure. We also provide a general inner bound in the case of limited common randomness.

==> Achievability/Q_1/convergence_in_probability_of_the_conditional_expected_distortion_for_Q_1.tex <==
\noindent ---------------------------------------------------------------------------
\subsection{Stronger property (but not necessary): convergence in probability}

Moreover, for $\mathbb{Q}_{\mathcal{C}^{(n)}}$-a.e. $c^{(n)}$ we have the following, where $\mathcal{L}_n$ denotes $[2^{n(R+\varepsilon)}] \times [2^{nR'}] \times [2^{nR_c}]$ and $\ell_n$ its cardinality $\lfloor 2^{n(R+\varepsilon)} \rfloor \lfloor 2^{nR'} \rfloor \lfloor 2^{nR_c} \rfloor:$
\begin{IEEEeqnarray}{rCl}
\IEEEeqnarraymulticol{3}{l}{
\mathbb{E}_{Q^{(1)}}[d(X^n,Y^n)|\mathcal{C}^{(n)}=c^{(n)}] \qquad \qquad
}\nonumber\\*
&=& \dfrac{1}{n} \sum_{k=1}^n \mathbb{E}_{Q^{(1)}}[d(X_k,Y_k)|\mathcal{C}^{(n)}=c^{(n)}] \nonumber \\*
&=& \dfrac{1}{n} \sum_{k=1}^n \sum_{(x,y) \in \mathcal{X}^2} d(x,y) \  \substack{\scalebox{1.0}{$Q^{(1)} \; (x^n, y^n)$\quad} \\ X^n, Y^n|\mathcal{C}^{(n)}=c^{(n)}} \nonumber \\*
&=& \dfrac{1}{n} \sum_{k=1}^n \sum_{(x,y) \in \mathcal{X}^2} d(x,y) \sum_{\substack{(m,m',j) \in \\ \mathcal{L}_n}} \dfrac{1}{\ell_n} \ \raisebox{2pt}{\scalebox{1.2}{$p$}} \substack{\scalebox{1.0}{$ (x, y) $} \\ \scalebox{0.7}{$X, Y|V\text{=}v_t(c^{(n)}, m, m', j)$} } \nonumber \\*
&=& \dfrac{1}{n} \sum_{k=1}^n \dfrac{1}{\ell_n} \sum_{(m,m',j) \in  \mathcal{L}_n} D(c^{(n)}, m, m', j, t) \label{eq:LLN_form}
\end{IEEEeqnarray}
where
$$D(c^{(n)}, m, m', j, t) = \sum_{(x,y) \in \mathcal{X}^2} d(x,y) \ \raisebox{2pt}{\scalebox{1.2}{$p$}} \substack{\scalebox{1.0}{$ (x, y) $} \\ \scalebox{0.7}{$X, Y|V\text{=}v_t(c^{(n)}, m, m', j)$} }.$$
By construction of $\mathcal{C}^{(n)},$ the variables $(D(\mathcal{C}^{(n)}, m, m', j, t))_{m,m',j,t}$ are independent and identically distributed. Their expectation is $\mathbb{E}_p[d(X,Y)].$ These variables are also bounded since $d$ is. Therefore, by the law of large numbers and \eqref{eq:LLN_form} we have
\begin{IEEEeqnarray}{c}
    \mathbb{E}_{Q^{(1)}}[d(X^n,Y^n)|\mathcal{C}^{(n)}]  \overset{\mathcal{P}}{\underset{n \to \infty}{\longrightarrow}} \mathbb{E}_p[d(X,Y)]. \label{eq:LLN_convergence}
\end{IEEEeqnarray}

We can then write almost sure inequalities using Lemma \ref{lemma:TV_continuity} and see all TV convergences with $Q_{\mathcal{C}, \cdot \cdot \cdot}$ as convergences in probability of the TV with $Q_{\cdot | \mathcal{C}}.$

\noindent ---------------------------------------------------------------------------


==> Achievability/Q_2 and P_1_2/old_Q_2.tex <==
\subsection{Distribution $Q^{(2)}$}
For every positive integer $n,$ define the following distribution:
\begin{IEEEeqnarray}{rCl}
\IEEEeqnarraymulticol{3}{l}{
Q^{(2)} \: (c^{(n)},m,m',j,v^n,x^n,y^n,z^n, \hat{m}')
}\nonumber\\* \quad
& = & Q^{(1)} \: (c^{(n)},m,m',j,v^n,x^n,z^n, \hat{m}') \nonumber \\*
&  & \scalebox{1.2}{$p$} \substack{\scalebox{0.95}{$ (y^n) \qquad \qquad \qquad \qquad \qquad \; \; $} \\ \scalebox{0.8}{$Y^n | Z^n=z^n, V^n=v^n(c^{(n)}, m,m',j)$} }.
\end{IEEEeqnarray}
Using the definition of $Q^{(1)}$ and the Markov property \eqref{eq:rates_region_Markov_long} we get:
\begin{IEEEeqnarray}{c}\label{eq:Q_2_X_Y_Z_knowing_V}
\substack{\scalebox{1.0}{$Q^{(2)} \; (x^n, y^n, z^n)$\quad} \\ X^n, Y^n, Z^n |V^n=v^n} = \prod_{t=1}^n \raisebox{2pt}{\scalebox{1.2}{$p$}} \substack{\scalebox{1.0}{$ (x_t, y_t, z_t) $} \\ \scalebox{0.7}{$X, Y, Z|V=v_t$} }.
\end{IEEEeqnarray}
% \begin{IEEEeqnarray}{rCl}
% \IEEEeqnarraymulticol{3}{l}{
% Q^{(2)} \: (c^{(n)},m,m',j,v^n,x^n,y^n,z^n, \hat{m'})
% }\nonumber\\* \quad
% & = & \mathbb{Q}_{\mathcal{C}^{(n)}}(c^{(n)}) \ \tfrac{\text{\normalsize 1}}{\lfloor 2^{nR} \rfloor \lfloor 2^{nR'} \rfloor \lfloor 2^{nR_c} \rfloor} \nonumber \\*
% &  & \substack{\scalebox{1.0}{$\mathbf{1} \qquad \qquad \qquad$}  \\ v^n = v^n(c^{(n)},m,m',j)} \ \prod_{t=1}^n p \substack{\scalebox{0.8}{$ (x_t, z_t) $} \\ \scalebox{0.55}{$X, Z|V=v_t$} } \, p \substack{\scalebox{0.8}{$(y_t)\qquad$} \\ \scalebox{0.55}{$Y|Z=z_t, V=v_t$} }\nonumber\\* \quad
% &  & \substack{\scalebox{1.0}{$P^D \; (\hat{m}') \qquad \qquad \quad $} \\ \hat{M}' | M=m, J=j, Z^n=z^n}\nonumber\\* \quad
% & = & \mathbb{Q}_{\mathcal{C}^{(n)}}(c^{(n)}) \ \tfrac{\text{\normalsize 1}}{\lfloor 2^{nR} \rfloor \lfloor 2^{nR'} \rfloor \lfloor 2^{nR_c} \rfloor} \nonumber \\*
% &  & \substack{\scalebox{1.0}{$\mathbf{1} \qquad \qquad \qquad$}  \\ v^n = v^n(c^{(n)},m,m',j)} \ \prod_{t=1}^n p \substack{\scalebox{0.8}{$ (x_t, y_t, z_t) $} \\ \scalebox{0.55}{$X, Y, Z|V=v_t$} }\nonumber\\* \quad
% &  & \substack{\scalebox{1.0}{$P^D \; (\hat{m}') \qquad \qquad \quad $} \\ \hat{M}' | M=m, J=j, Z^n=z^n},
% \end{IEEEeqnarray} where the last equality uses the Markov property $X-Z,V-Y$ in \eqref{eq:def_S}.
Hence, the following marginals match: $Q^{(2)}_{\mathcal{C}^{(n)}, M, M', J, V^n, Y^n, \hat{M}'} \equiv Q^{(1)}_{\mathcal{C}^{(n)}, M, M', J, V^n, Y^n, \hat{M}'}$ and $Q^{(2)}_{\mathcal{C}^{(n)}, M, M', J, V^n, X^n, Z^n, \hat{M}'} \equiv Q^{(1)}_{\mathcal{C}^{(n)}, M, M', J, V^n, X^n, Z^n, \hat{M}'}$. In particular $Q^{(2)}_{\mathcal{C}^{(n)}, Y^n} \equiv Q^{(1)}_{\mathcal{C}^{(n)}, Y^n}$ and $Q^{(2)}_{\mathcal{C}^{(n)}, J, X^n, Z^n} \equiv Q^{(1)}_{\mathcal{C}^{(n)}, J, X^n, Z^n},$ hence by \eqref{eq:TV_Q_1_Y} and \eqref{eq:TV_Q_1_X_Z} we have
\begin{equation}\label{eq:TV_Q_2_Y}
    \mathbb{E}_{\mathcal{C}^{(n)}}\big[\|Q^{(2)}_{Y^n|\mathcal{C}^{(n)}=\cdot} - p_{Y}^{\otimes n}\|_{TV}\big] \underset{n \to \infty}{\longrightarrow} 0 \text{ and}
\end{equation}
\begin{equation}\label{eq:TV_Q_2_X_Z}
    \forall j, \quad \mathbb{E}_{\mathcal{C}^{(n)}}\big[\|Q^{(2)}_{X^n, 
Z^n|\mathcal{C}^{(n)}=\cdot, J=j} - p_{X, Z}^{\otimes n}\|_{TV}\big] \underset{n \to \infty}{\longrightarrow} 0.
\end{equation}

==> Other sections/Unused files/Failed_Markov_inequality_attempt.tex <==
We start by exhibiting an event on which the average distortion criterion is satisfied.
From \eqref{eq:Distortion_P}, there exists a positive integer $N_0$ such that for all $n>N_0$ we have $$\mathbb{E}_{P}[d(X^n,Y^n)] \leq \Delta - \tfrac{\varepsilon}{2}, \text{ i.e. }$$ 
\begin{IEEEeqnarray}{c}\label{eq:expect_before_Markov_ineq}
    \mathbb{E}_{\mathcal{C}^{(n)}}\big[ \mathbb{E}_{P_{X^n,Y^n|\mathcal{C}^{(n)}=\cdot}} [d(X^n,Y^n)] \big] \leq \Delta - \tfrac{\varepsilon}{2}.\IEEEeqnarraynumspace
\end{IEEEeqnarray}
For every $n \geq 1$ we define the following deterministic real-valued function $$ e_n : c^{(n)} \mapsto \mathbb{E}_{P_{X^n,Y^n|\mathcal{C}^{(n)}=c^{(n)}}} [d(X^n,Y^n)] .$$ Since $e_n \geq 0$ we can use the Markov inequality then use \eqref{eq:expect_before_Markov_ineq}: for all $n>N_1,$
\begin{IEEEeqnarray}{c}
    \mathbb{Q}_{\mathcal{C}^{(n)}}(e_n(\mathcal{C}^{(n)}) \leq \Delta) \geq  1 - \dfrac{\mathbb{E}_{\mathcal{C}^{(n)}}[e_n(\mathcal{C}^{(n)})]}{\Delta } \geq 1 - \dfrac{\Delta - \tfrac{\varepsilon}{2}}{\Delta} \geq \dfrac{\varepsilon}{2\Delta}.\IEEEeqnarraynumspace
\end{IEEEeqnarray}
We now exhibit a second and very probable event on which a perception constraint is satisfied. We fix $\delta>0.$\\
We define the following deterministic real-valued function $$ h_n : c^{(n)} \mapsto \|P_{Y^n|\mathcal{C}^{(n)}=\cdot} - p_{Y}^{\otimes n}\|_{TV} .$$ Since $h_n \geq 0$ the convergence in \eqref{eq:TV_P_Y} is a $L^1$ convergence, which implies the convergence in probability. Therefore, there exists a positive integer $N_{\delta}$ such that for all $n>N_{\delta}$ we have
\begin{IEEEeqnarray}{c}
    \mathbb{Q}_{\mathcal{C}^{(n)}}(h_n(\mathcal{C}^{(n)}) \leq \delta) \geq  1 - \dfrac{\varepsilon}{2\Delta}.\IEEEeqnarraynumspace
\end{IEEEeqnarray}
YES BUT NOT NECESSARILY GOING TO ZERO AS FAST AS $(2^{-nH_p(V)})^{2^{n(R+R'+R_c)}},$ which the probability of a codebook having only $p_V-$typical codewords.

UNLESS IMPROVE SOFT COVERING LEMMA TO GET A SPEED WHICH IS LIKELY TO NOT BE AS BAST AS $2^{2^n}$!!

For a distribution $P$ the use of a random variable name as a subscript such as in $P_X$ denotes the marginal

==> Other sections/Unused files/scalebox_attempts.tex <==
\begin{align}\label{eq:def_S_D_infty}
      & 
    \left\{ \begin{array}{rcl}
    \scalebox{0.90}{$(R, \Delta) \in \mathbb{R}_{\geq 0}^2$} &:& \scalebox{0.85}{$\exists \ p_{X,Z,V,Y} \in \mathcal{D}_D \text{ s.t. }$} \\
        \scalebox{0.85}{$R$} &\geq& \scalebox{0.85}{$I_p(X;V|Z)$} \\
        \scalebox{0.85}{$\Delta$} &\geq& \scalebox{0.85}{$\mathbb{E}_p[d(X, Y)]$}
    \end{array}\right\}, 
\end{align}
where $\mathcal{D}_D$ is defined as
\begin{align}\label{eq:def_D_D}
       & 
    \left\{ \begin{array}{rcl}
        &\scalebox{0.85}{$p_{X,Z,V,Y} : (X,Z) \sim p_{X,Z}$}& \\
        &\scalebox{0.85}{$p_{Y} \equiv p_{X}$}&\\
        &\scalebox{0.85}{$Z - X - V$}& \\
        &\scalebox{0.85}{$X - (Z, V) - Y$}& \\
        &\scalebox{0.85}{$I_p(Z;V) < \infty$}&
        %\exists \nu \ \sigma\text{-finite s.t. }& p \ll & \mu \times \gamma \times \nu \times \mu
    \end{array}\right\},
\end{align}
